ESDIRK-based nonlinear model predictive control for stochastic differential-algebraic equations

In this paper, we present a nonlinear model predictive control (NMPC) algorithm for systems modeled by semi-explicit stochastic differential-algebraic equations (DAEs) of index 1. The NMPC combines a continuous-discrete extended Kalman filter (CD-EKF) with an optimal control problem (OCP) for setpoint tracking. We discretize the OCP using direct multiple shooting. We apply an explicit singly diagonal implicit Runge-Kutta (ESDIRK) integration scheme to solve systems of DAEs, both for the one-step prediction in the CD-EKF and in each shooting interval of the discretized OCP. The ESDIRK methods use an iterated internal numerical differentiation approach for precise sensitivity computations. These sensitivities are used to provide accurate gradient information in the OCP and to efficiently integrate the covariance information in the CD-EKF. Subsequently, we present a simulation case study where we apply the NMPC to a simple alkaline electrolyzer stack model. We use the NMPC to track a time-varying setpoint for the stack temperature subject to input bound constraints.

==> tex/introduction.tex <==
\section{Introduction}
\label{sec:Introduction}

Nonlinear model predictive control (NMPC) algorithms are widely used in the control of chemical systems to optimize economics or minimize deviations from setpoints \cite{Ritschel:Joergensen:2019}. An NMPC algorithm is a feedback control strategy that applies the solutions from optimal control problems (OCPs) based on a mathematical model of the system in a moving horizon fashion. Since chemical systems are best modeled using differential-algebraic equations (DAEs) \cite{Biegler:etal:2012}, it follows that the models employed in NMPC strategies should also incorporate DAEs. 

Implementing the OCPs using a direct multiple-shooting approach requires numerical integration schemes to solve initial-value problems (IVPs) for DAEs. Software solutions for solving IVPs for DAEs include the codes DASSL, which utilizes a backward differentiation formula (BDF), and RADAU5, employing a 3-stages fully implicit Runge-Kutta (IRK) integration scheme \cite{Ascher:Petzold:1998}. Due to the frequent discontinuities inherent in multiple-shooting-based NMPC, BDF methods may experience frequent restarts, leading to a reduction in integration order \cite{Kristensen:etal:2004}. In contrast, the fully implicit IRK methods do not suffer from the reduction of integration order. However, these methods are in general considered computationally expensive methods as they require the solution of large systems of nonlinear equations in each integration step. Therefore, the diagonal IRK methods, such as explicit singly diagonal implicit Runge-Kutta (ESDIRK) integration schemes, offer a computationally efficient alternative. ESDIRK methods, characterized by identical coefficients in the diagonal of their Butcher tableaus and with the first step being explicit, enable the reuse of matrix factorizations across stages, thereby enhancing computational efficiency in solving IVPs for DAEs. 

Solving the OCPs also requires integrator sensitivity information. Equipping the implementation of the ESDIRK integration schemes with iterated sensitivity computations based on the principle of internal numerical differentiation (IND), ensures precise sensitivity information. The principle
of IND involves computing the sensitivities by directly differentiating the discretization scheme generated adaptively
from the integrator \cite{Bock:1981, Albersmeyer:2010}. \cite{Andersen:Joergensen:2023} present such sensitivities for the ESDIRK methods applied to ODEs.

In practical applications, solving the OCPs requires frequent updates of the full-state information of the system. State estimators, such as Kalman filters, compute this information based on noisy measurements and models representing the plant-model mismatch. Consequently, state estimators play a crucial role in the successful implementation of NMPC for physical systems. The extension of DAEs with stochastic processes provides a means to account for this plant-model mismatch.

In this paper, we consider the continuous-discrete semi-explicit stochastic DAE (SDAE) systems of the form
\begin{subequations}
\label{eq:SDAE_model_w_meas_and_output_eqs}
\begin{alignat}{2}
    dx(t) &= f(t, x(t), y(t), u(t), d(t))dt + \sigma d\omega(t), \label{subeq:SDE}\\
    0 &= g(t, x(t), y(t), u(t), d(t)),\\
    y_k^m &= m(t_k, x_k, y_k, u_k, d_k) + v_k,\label{subeq:meas_eq}\\
    z(t) &=  h(t, x(t), y(t), u(t), d(t)) \label{subeq:out_eq},
\end{alignat}
\end{subequations}
where $t$ is time, $x(t)$ is the vector of differential states, $y(t)$ is the vector of algebraic states, $u(t)$ is the vector of inputs, and $d(t)$ is the vector of disturbances.
$\omega(t)$ is a standard Wiener process, i.e., $d\omega(t) \sim N_{iid}(0, Idt)$, representing the plant-model mismatch and $v_k \sim N_{iid}(0, R_k)$ is the measurement noise with $R_k$ being the covariance. $y_k^m = y^m(t_k)$ represent the measurements at the time $t_k$ and $z(t)$ is the output of the model. 

We demonstrate how to implement an NMPC algorithm for systems described by \eqref{eq:SDAE_model_w_meas_and_output_eqs} of index-1. The NMPC algorithm combines a continuous-discrete extended Kalman filter (CD-EKF) and an OCP for setpoint tracking. We use a direct multiple shooting approach for transcribing the OCP into a nonlinear programming (NLP) problem that we solve using a sequential quadratic programming (SQP) solver.
We demonstrate how to apply the ESDIRK methods with iterated sensitivity generation in both the CD-EKF and the OCP. In this context, we use the sensitivity information to compute the gradient information in the OCP and to calculate the covariance in the CD-EKF.
We test the NMPC algorithm on a numerical case study of an alkaline electrolyzer stack affected by a stochastic process. We use the NMPC to track a time-varying setpoint for the temperature in the stack. 

The main novelty in this paper is the direct demonstration of how ESDIRK integration schemes with IND-based sensitivities computations can be applied to address both the state estimation problem and the OCP, resulting in a unified NMPC solution for DAEs.

The rest of the paper is structured as follows. Section \ref{sec:simulation_and_sensitivity_gen} describes the ESDIRK integration scheme used for solving the IVPs of DAEs in both CD-EKF and OCP. We derive iterated IND sensitivities for these ESDIRK methods, and we introduce an implicit-explicit scheme for solving the IVPs for SDAE systems. In Section \ref{sec:NMPC}, we introduce the NMPC and demonstrate how to implement the CD-EKF and OCP for index-1 semi-explicit DAEs. Section \ref{sec:case_study} presents a case study using the model of an alkaline electrolyzer stack. Section \ref{sec:conclusions} concludes the paper.

==> tex/old.tex <==
\begin{subequations}
\label{eq:OCP2}
\begin{alignat}{4}
       & && \min_{x,y,u} \phi_k,&&& \\
       & \mathrm{s.t.} \quad && x(t_k) = \hat{x}_{k|k},&&&  \\
       & && \frac{dx(t)}{dt} = f(t, x, y, u, d),  t\in [t_k, \, t_k+T_N],&&&\\
       & && 0 = g(t, x, y, u, d),  t\in [t_k, \, t_k+T_N],&&& \\
       & && z(t) = h(t, x, y, u, d), &&& \label{subeq:output_equation}\\ 
       & && u(t) = u_{k+j},  t\in [t_{k+j}, \, t_{k+j+1}],  \quad j \in \mathcal{N},&&&\\
       & && d(t) = d_{k+j},  t\in [t_{k+j}, \, t_{k+j+1}],  \quad  j \in \mathcal{N},&&& \label{subeq_dist_j}\\
       & && u_{\min} \leq u_{k+j} \leq u_{\max},  \qquad \qquad \quad \, j \in \mathcal{N},&&&
\end{alignat}
\end{subequations}


\begin{equation}
    \phi_{z,k,j} = \frac{1}{2}\int_{t_j}^{t_{j+1}}\left \|  z_j(t)-\Bar{z}_j(t)\right \|_{Q_{z}}^2dt,
\end{equation}
such that $\phi_{z,k} = \sum_{j=0}^{N-1}  \phi_{z,k,j}$. We do this by formulating the integrals as IVPs and solving them simultaneously with \eqref{eq:relaxed_DAE}. The transcribed OCP as the NLP
\begin{subequations}
\label{eq:NLP_OCP}
\begin{alignat}{4}
      & && \min_{\{x_{k+j+1}, y_{k+j}, u_{k+j}\}_{j=0}^{N-1}} \phi_k(\{x_{k+j+1}, y_{k+j}, u_{k+j}\}_{j=0}^{N-1},&&& \\
       & &&s.t. \quad  x_k = \hat{x}_{k|k},&&&  \\
       & && x_{k+j+1} = F(x_{k+j}, y_{k+j}, u_{k+j}), \quad \, j \in \mathcal{N}, \label{subeq:continuity} &&&\\
       & && 0 = g(x_{k+j}, y_{k+j}, u_{k+j}),\qquad \qquad j \in \mathcal{N}, &&& \label{subeq:consistency} \\
       & && u_{\min} \leq u_{k+j} \leq u_{\max},\qquad \qquad \quad \; j \in \mathcal{N}. &&&
\end{alignat}
\end{subequations}

$F(\cdot)$ represents ESDIRK integration scheme for solving \eqref{eq:relaxed_DAE} at initial conditions ($x_{k+1}, y_{k+j}$).
Eq. \eqref{subeq:continuity} is the continuity constraints and we apply \eqref{subeq:consistency} to ensure consistency of the algebraic equations at the beginning of each shooting interval.  We use the filtered algebraic state to initialize $y_k = \hat{y}_{k|k}$. The NLP in \eqref{eq:NLP_OCP} has the decision variables $w = (x_k, y_k, u_k, x_{k+1}, y_{k+1}, u_{k+1} \dots, u_{k+N-1}, x_{k+N})$, and we denote the equality constraints \eqref{subeq:continuity}-\eqref{subeq:consistency} as $b(w)$.
The gradient of the $b(w)$, $\frac{\partial b(w)}{\partial w}$, related to \eqref{subeq:continuity} requires the sensitivities $ \frac{\partial F}{\partial x_{k+j}}$, $\frac{\partial F}{\partial y_{k+j}}$, and $\frac{\partial F}{\partial u_{k+j}}$,
which we obtain by computing the iterated IND sensitivities. The gradients related to \eqref{subeq:consistency} are calculated by evaluating the Jacobians. 
